Broadband characterisation of the very intense TeV flares of the blazar 1ES 1959+650 in 2016

1ES 1959+650 is a bright TeV high-frequency-peaked BL Lac object exhibiting interesting features like "orphan" TeV flares and a broad emission in the high-energy regime, that are difficult to interpret using conventional one-zone Synchrotron Self-Compton (SSC) scenarios. We report the results from the Major Atmospheric Gamma Imaging Cherenkov (MAGIC) observations in 2016 along with the multi-wavelength data from the Fermi Large Area Telescope (LAT) and Swift instruments. MAGIC observed 1ES 1959+650 with different emission levels in the very-high-energy (VHE, E >100 GeV) gamma-ray band during 2016. In the long-term data, the X-ray spectrum becomes harder with increasing flux and a hint of a similar trend is also visible in the VHE band. An exceptionally high VHE flux reaching ~ 3 times the Crab Nebula flux was measured by MAGIC on the 13th, 14th of June and 1st July 2016 (the highest flux observed since 2002). During these flares, the high-energy peak of the spectral energy distribution (SED) lies in the VHE domain and extends up to several TeV. The spectrum in the gamma-ray (both Fermi-LAT and VHE bands) and the X-ray bands are quite hard. On 13th June and 1st July 2016, the source showed rapid variations of the VHE flux within timescales of less than an hour. A simple one-zone SSC model can describe the data during the flares requiring moderate to high values of the Doppler factors (>=30-60). Alternatively, the high-energy peak of the SED can be explained by a purely hadronic model attributed to proton-synchrotron radiation with jet power L_{jet}~10^{46} erg/s and under high values of the magnetic field strength (~100 G) and maximum proton energy (~few EeV). Mixed lepto-hadronic models require super-Eddington values of the jet power. We conclude that it is difficult to get detectable neutrino emission from the source during the extreme VHE flaring period of 2016.

==> Results/TBL_SED_1ES1959+650_2016_peaks_LAT.tex <==
\begin{table*}
\caption{Fitting parameters of the high-energy gamma-ray spectrum during the highest-flux nights}
\label{tb:SED_FitParameters_LAT}
\centering  
\begin{tabular}{c|cccc}
Date & Fit model & Flux\tablefootmark{a} & Differential flux density\tablefootmark{b} & $\Gamma$ \\ 
& & $\mathrm{(cm^{-2}\cdot s^{-1})}$ & $\mathrm{(MeV^{-1} cm^{-2}\cdot s^{-1}})$ & \\ \hline
21:00 12th--09:00 14th June & & \\
 (MJD 57551.875--57553.375) & PL & $(9.6 \pm 3.0)\times 10^{-8}$ & $(9.8 \pm 2.9)\times 10^{-12}$ & $1.57 \pm 0.20$ \\ % \hline
\end{tabular}
\tablefoot{The function PL is defined in Sec.\ref{ssec:ObsAna:MAGIC}. The normalization energy $E_0$ is 1.96 GeV.}
\tablefoottext{a}{For an energy range 0.3--300 GeV.}
\tablefoottext{b}{At the normalization energy 1.96 GeV.}
\end{table*}

==> Results/TBL_SED_1ES1959+650_2016_peaks_XRT.tex <==
\begin{table*}
\caption{Fitting parameters of the X-ray spectra during the highest-flux nights}
\label{tb:SED_FitParameters_XRT}
\centering  
\begin{tabular}{c|ccccccc}
Date & Fit model & \multicolumn{2}{c}{Flux $\mathrm{(erg \cdot cm^{-2} \cdot s^{-1})}$} & $\Gamma \,\rm{or} \,\alpha$ & $\beta$ & $\chi^2/d.o.f$ \\
%& & \multicolumn{2}{c}{$\mathrm{(erg \cdot cm^{-2} \cdot s^{-1})}$} & & & \\
{   } & {   } & 2--10 keV & 0.5--5 keV & {} & {} & {} \\
\hline
02:47--03:57 13th June & PL & $4.35_{-0.07}^{+0.07}\times 10^{-10}$ & $5.15_{-0.04}^{+0.04}\times 10^{-10}$ & $$1.81_{-0.01}^{+0.01}$$ & \cdots & $0.921$ \\[1.2ex]
{(MJD 57552.116--57552.165)}& LogP & $4.39\times 10^{-10}$ &$5.15\times 10^{-10}$ & $$1.83_{-0.03}^{+0.03}$$ & $$-0.03_{-0.04}^{+0.04}$$ & $0.922$ \\[1.2ex] \hline

02:18--02:33 14th June & PL & $4.88_{-0.08}^{+0.08}\times 10^{-10} & 5.84_{-0.05}^{+0.05}\times 10^{-10}$ & $1.82_{-0.01}^{+0.01}$ & \cdots & $1.11$ \\[1.2ex]
{(MJD 57553.096--57553.106)}& LogP & $4.91\times 10^{-10}$ & $5.84\times 10^{-10}$ & $1.84_{-0.03}^{+0.03}$ & $-0.02_{-0.04}^{+0.04}$ & $1.11$ \\[1.2ex]%\hline
\end{tabular}
\tablefoot{The function PL and LogP are defined in Sec.\ref{ssec:ObsAna:MAGIC}. \textbf{The normalization energy is fixed at 1 keV.} The uncertainty of the flux is not provided for the log-parabola.}
%\tablefoottext{a}{Only $E_{peak}$ is determined by an independent fitting with log-parabola which is expressed by $E_{peak}$ and $\beta$~at $E_{peak}$.}
\end{table*}

==> hidden.tex <==
%@arxiver{FIG_LightCurve_1ES1959+650_MWL_2016_months.pdf,SSC_13June.png,13June_10mins_300GeV_LC.png}
